Trapping LLM Hallucinations Using Tagged Context Prompts

Recent advances in large language models (LLMs), such as ChatGPT, have led to highly sophisticated conversation agents. However, these models suffer from "hallucinations," where the model generates false or fabricated information. Addressing this challenge is crucial, particularly with AI-driven platforms being adopted across various sectors. In this paper, we propose a novel method to recognize and flag instances when LLMs perform outside their domain knowledge, and ensuring users receive accurate information. We find that the use of context combined with embedded tags can successfully combat hallucinations within generative language models. To do this, we baseline hallucination frequency in no-context prompt-response pairs using generated URLs as easily-tested indicators of fabricated data. We observed a significant reduction in overall hallucination when context was supplied along with question prompts for tested generative engines. Lastly, we evaluated how placing tags within contexts impacted model responses and were able to eliminate hallucinations in responses with 98.88% effectiveness.

==> text/discussion.tex <==
\section{Discussion}

Context prompting is a more reliable way of getting accurate, timely results to the user. PerplexityAI seems to have figured this out (Figure~\ref{fig:perplexity}):

\begin{figure} [htb]
    \centering
    \fbox{\includegraphics[width=0.75\textwidth]{figures/perplexity}}
    \caption{PerplexityAI found me in a 3-day old blog post (viztales.com)!}
    \label{fig:perplexity}
\end{figure}

It is also a good way to make and AI app more jailbreak resistant by requiring tagged sources to be present in the response. By filtering out or changing the source tags, it should be able to thwart jailbreaks that derive the context (in this case tags)

It seems reasonable at this point to explore if, rather then creating ever-larger models that \enquote{memorize} all the correct information, we instead take a different approach. Focus on two elements:

\begin{enumerate}
    \item Continue the focus on embeddings for finding relevant data. This can be applied lake a search engine to trustworthy sources or conspiracy swamps alike. But the user will have agency in the choice of what information they see
    \item Emphasize effective summarizing at levels of abstraction for question-answering LLMs. It may be that these models don't need to know much, they just need to write well.
\end{enumerate}

To provide some support for this argument, compare the response from the Curie-instruct-beta to the question \enquote{\textit{How can technology be utilized to effectively introduce diversity injection techniques into various social networks?}} without context prompting and then with. When provided no context, the Curie model provides a useless, almost incoherent response. But when provided with context, it provides a ChatGPT-level response:

\paragraph{No context:}
\begin{displayquote}
    \textit{Diversity injection techniques can be introduced by employing the use of new media (such as social media). Web 2.0 tools can be utilized to interact with various stakeholders and introduce the concepts of workforce diversity. Additionally, organizations can broadcast news and promotional materials to target different audiences, creating a diverse and inclusive atmosphere.}

    \textit{The use of social media technology can be used to introduce injection into various social networks. Diversity injection can also be conducted by using different types of media to target different audiences. For example, a company could post news and promotional materials to different social media platforms to reach different audiences and introduce diversity throughout the workforce.}
\end{displayquote}

\paragraph{Tagged context}
\begin{displayquote}
    \textit{Technology can be utilized to introduce diversity injection techniques into various social networks by promoting diverse information instead of suppressing it. This can break down the walls that create conditions for belief stampedes. The use of newsletters, talks, and online forums can be used to provide individuals with access to diverse information and social groups they may not encounter otherwise . By targeting individuals with latent interests that may fill the same needs as belonging to a cult, diversity injection can work one person at a time, nudging them off the stampede trajectory . Social media platforms can also be used to promote diverse perspectives and reduce polarization by introducing diversity into social networks . By creating resilient ecosystems that resist belief stampedes, diverse communities can be formed using technology to improve our ability to understand differing beliefs and perspectives . Therefore, technology can be effectively utilized to introduce diversity injection techniques into various social networks by promoting diverse information and creating resilient ecosystems that resist belief stampedes.}
\end{displayquote}

Although not quite as refined and sophisticated as the ChatGPT (try it out!) or GPT-4, this is a very effective response and one that contains no hallucinations. 

These results imply directions for future work, where prompt and language model are considered together as a mechanism for producing trustworthy answers to questions. Some directions for future research might include:

\begin{itemize}
    \item Most fundamentally, is the question answering a different branch for LLMs? Models such as the GPT have become much more than question answering systems. They are used to assist in writing, editing, software development, and producing poems on demand. Would a set of more specialized, smaller models be more useful than giant models such as the GPT-4? Or are the emergent properties that appear to be correlated with scale worth the effort and cost to produce them\footnote{The GPT-4 is apparently as good at writing code as the more specialized Codex model according to conversations with Microsoft engineers.}? There is substantial work in developing specialized models for particular domains, such as BioMedGPT~\cite{zhang2023biomedgpt}, and the notorious Galactica~\cite{taylor2022galactica}, a large language model for science that hallucinated wildly and was available online for only three days~\cite{heaven2022meta}.
    \item What are the bounds for an optimal context-based question-answering model? Are there different architectures and training techniques that would emphasize organization and presentation of answers from corpora?
    \item What are the bounds for an optimal context prompt? Prompts are surprisingly complex structures that adapt to their development and the input of the user. History, variability, even dynamic retroactive updating of the ongoing prompt should be explored
    \item How should context prompts be produced? The idea of using embeddings to search the domain is remarkably effective in producing a context that the model is able to use. But it may be possible to search multiple domains and produce more sophisticated contexts in ways that produce higher-quality answers. For example, in this work, we produced summaries that traced back to the original text. This allowed the LLM (GPT-3.5-turbo) to \enquote{average out} text like figure captions and footnotes. It also provided the capability of producing a \endquote{rolling window} of overlapping summaries to aid in the embedding search.
    \item Attribution. When a model is trained on data, it often is unable to point in a meaningful way to the data that it used to produce its response. Even in the case where a citation is accurately provided and not hallucinated, the \textit{source} for that citation may be another work that is not acknowledged in the result. This is profoundly unethical, and could destroy the business model for many sites who provide information in return for paying subscribers or being able to present advertising to users. 
    \item What are the ethical implications of such an approach? In this role, the LLMs contribution is limited to the organization of the information in the context and the production of high-quality text. What if the corpora used to produce the context is entirely made up of mass-shooter manifestos? Should that be detected? If so, what should the response be? After all, the user may be a researcher, trying to uncover patterns in otherwise reprehensible documents. Lastly, what does it mean to produce \enquote{High-quality text?} What languages and dialects get the requisite training data and which do not? Or can a system be trained to pick up the textual patterns from the corpora being searched. In our experiences using the King James Bible and Moby-Dick, it certainly seems like this is a side effect of this approach. Is it desirable?
\end{itemize}

The way that many of us use computers changed on November 30, 2022, when OpenAI released ChatGPT. The implications of LLMs that are easily mistaken for intelligent, trustworthy agents has suddenly become a pressing issue. Producing truly trustworthy systems that are capable of responding to new information without requiring continuous (expensive!) retraining is essential to being able  to produce an accountable role for computer-human interactions with what we now call AI.

\begin{comment}
Compare this to the response generated by the GPT-4.:

\begin{displayquote}
    \textit{Technology can be utilized to effectively introduce diversity injection techniques into various social networks by promoting diverse information instead of suppressing it. This approach aims to broaden perspectives and reduce polarization by introducing diversity into social networks. By using technology, such as social media platforms or newsletters, to target individuals with latent interests that may fill the same needs as belonging to a cult, diversity injection can disrupt belief stampedes. The goal is not to change everyone's behavior around dangerous misinformation, but rather to break off small segments from an existing belief stampede, making it less dangerous. This can be done by nudging individuals off the trajectory of a stampede into a world where they have more freedom to move. Diverse communities create resilient ecosystems that resist belief stampedes, and technology can help in creating such communities. By exposing individuals to reality-based information and social groups they would not encounter otherwise, diversity injection can remove individuals from misinformation streams. Over time, the belief distance may grow great enough that it no longer makes sense to them. This approach works one person at a time, but with enough members nudged from the path of a belief stampede, the group as a whole has to adjust its narrative or risk disintegration. Technology can be a powerful tool in introducing diversity injection techniques into various social networks and breaking down the walls that create conditions for stampedes in the first place.}
\end{displayquote}

Both are readable and largely accurate, but the second may be too verbose to make an effective point. Regardless, the similarities in capability are striking even though one model is a fraction of the size of the other.
\end{comment}
